Curly Flow Matching for Learning Non-gradient Field Dynamics

Modeling the transport dynamics of natural processes from population-level observations is a ubiquitous problem in the natural sciences. Such models rely on key assumptions about the underlying process in order to enable faithful learning of governing dynamics that mimic the actual system behavior. The de facto assumption in current approaches relies on the principle of least action that results in gradient field dynamics and leads to trajectories minimizing an energy functional between two probability measures. However, many real-world systems, such as cell cycles in single-cell RNA, are known to exhibit non-gradient, periodic behavior, which fundamentally cannot be captured by current state-of-the-art methods such as flow and bridge matching. In this paper, we introduce Curly Flow Matching (Curly-FM), a novel approach that is capable of learning non-gradient field dynamics by designing and solving a Schr\"odinger bridge problem with a non-zero drift reference process -- in stark contrast to typical zero-drift reference processes -- which is constructed using inferred velocities in addition to population snapshot data. We showcase Curly-FM by solving the trajectory inference problems for single cells, computational fluid dynamics, and ocean currents with approximate velocities. We demonstrate that Curly-FM can learn trajectories that better match both the reference process and population marginals. Curly-FM expands flow matching models beyond the modeling of populations and towards the modeling of known periodic behavior in physical systems. Our code repository is accessible at: https://github.com/kpetrovicc/curly-flow-matching.git

==> NeurIPS_2025_Template/old/01introduction.tex <==
\section{Introduction}
\label{01introduction}
Understanding temporal evolution of multi-body systems remains a central challenge across life sciences domain~\citep{lange2024mapping, pan2024studying}, as such systems are often characterized by complex internal dynamics governing their evolutionary behavior. For example, in biomedical domain--e.g tissue, system evolves through tissue differentiation characterized by cell divisions and deaths as well as morphological changes. Learning evolutionary behavior in such systems can be formulated as a \textbf{trajectory inference} problem~\citep{pmlr-v48-hashimoto16, lavenant2023mathematicaltheorytrajectoryinference}, where the goal is to recover full trajectories of particles in a system over the observed time period. 

Inferring particle trajectories remains a core challenge in experimental setting, especially in the case of RNA single-cell sequencing which is known to be highly expensive and destructive to the sample, thereby proving to be unideal for inferring continuous cell trajectories over time and motivating development of more prominent computational frameworks.

Trajectory inference has been studied by current prominent flow matching frameworks such as: Generalized Schr{\"o}dinger Bridge Matching~\citep{liu2024generalizedschrodingerbridgematching} and Wasserstein Lagrangian Flows~\citep{neklyudov2024computationalframeworksolvingwasserstein}. However, none of the current methods account for complex motion patterns such as rotation, turbulence and chaos which arise as a result of non-gradient field dynamics. These patterns appear to be particularly important in my real-world systems. For example, in tumour tissue, cells can form cell cycles~\citep{riba2022cell} as a result of adhesive forces~\citep{wirtz2011physics} and signaling inducing rotational motion that significantly impacts their trajectories. Another prominent example is weather forecasting~\citep{lam2022graphcast}, where turbulent flow significantly impacts fluid particle trajectory. 

A natural question arises: \textit{How can we improve current flow matching set-up to model complex motion patterns in data?}

% Flow-based models have been utilized to learn cell trajectories~\cite{kapuśniak2024metricflowmatchingsmooth, tong2024improvinggeneralizingflowbasedgenerative, tong2020trajectorynetdynamicoptimaltransport}, primarily focusing on learning the velocity-field of particles (cells) in the system (tissue). However, it has been shown that system dynamics is impacted by internal interactions, such is \textit{cell signaling}~\cite{armingol2021deciphering, goodenough2009gap} or \textit{fusing}~\cite{shultes2024cell}
% resulting in significant influence over cell trajectories and alterations in tissue structure. Such interactions are often neglected resulting in inaccurate trajectory inference and representation of system dynamics. Recent work by~\cite{atanackovic2024meta} and ~\cite{neklyudov2023actionmatchinglearningstochastic} show the impact of intercellular interactions to infer their trajectories, setting a new paradigm for trajectory inference.

In this work, we propose \textit{Schr{\"o}dinger Bridge Matching with Solenoidal Constraints}, a novel generative modeling paradigm that models probability flow leveraging non-gradient field dynamics arising from intrinsic forces in the empirical data. We do so by introducing a force-field component in addition to curl-free field. 

==> NeurIPS_2025_Template/old/02background.tex <==
\section{Theoretical background and motivation}
\label{section 02}
\subsection{Generative Modeling via Flow Matching}
\label{section 02.1}
Flow matching \cite{lipman2023flowmatchinggenerativemodeling} is a powerful generative modeling framework which concerns finding probability paths or \textit{flows} that connect source $p_0(x_0)$ and target $p_1(x_1)$ distribution by computing a map $f_t$ such that $f_t: p_0 \rightarrow p_1$.

Let us consider a source distribution $p_0$ and target distribution $p_1$ for which we draw samples $x_0 \sim p_0(x_0)$ and $x_1 \sim p_1(x_1)$, such that $(x_0, x_1)$ is coupled by joint distribution $\pi_{x_0, x_1} = p_0(x_0)p_1(x_1)$. The interpolant $x_t$ between $x_0$ and $x_1$ can be interpreted by computing a map $f_t$ as:
\looseness=-1
\begin{equation}
    x_t = f_t(x_0, x_1), \quad (x_0, x_1) \sim \pi_{x_0, x_1},
\end{equation} 
\looseness=-1
where $f_t$ is a continuous interpolating map defined on interval $t \in [t_0, t_1]$ for which it holds that $f_{t=t_0}(x_0, x_1)=x_0$ and $f_{t=t_1}(x_0, x_1)=x_1$. For example, $f_t$ could be a linear mapping between $x_0$ and $x_1$ such that $x_t = (1-t) \cdot x_0 + t \cdot x_t$.
\subsection{Schr{\"o}dinger Bridge Matching}
% \subsection{Manifold Flow Matching}
% \label{section 02.2}
% Let $(\mathcal{M},g)$ be a smooth orientable manifold supported by a smooth map $g$, where a tangent space for a point $x$ on manifold $\mathcal{M}$ is assigned by an inner product $\langle.,.\rangle_{g}$ at $x$. We consider paths $\gamma_t$ on manifold $(\mathcal{M},g)$, which connect points $x_0$ and $x_1$ drawn from a joint distribution such that $(x_0, x_1) \sim \pi_{x_0, x_1}$.
% \begin{equation}
%     \gamma_t^* = \text{arg min}_{\gamma_t} \int \dot \gamma_t^T G(\gamma_t, \mathcal{D}) \dot \gamma_t dt
% \end{equation}
% s.t.\ $\gamma_0 = x_0$ and $\gamma_1 = x_1$.

% \subsection{Multi-body System Dynamics}
% \label{section 02.3}

% \xhdr{Mean-field Limit of Interacting Particles}
% \begin{equation}
%     \frac{dx}{dt} = \mathbb{E}_{p_t(y)} k(x, y), \quad \frac{\partial p_t(x)}{\partial t} = - \langle \nabla_x, p_t(x) \mathbb{E}_{p_t(y)} k(x,y) \rangle
% \end{equation}

% \begin{equation}
%     V(p_t, v_t) = 
% \end{equation}



% \xhdr{Principle of Minimal Action}

==> NeurIPS_2025_Template/old/03framework.tex <==
\section{Problem Formulation}
\label{02problemformulation}
Existing flow-based models~\citep{lipman2023flowmatchinggenerativemodeling, liu2024generalizedschrodingerbridgematching} model particles evolving according to a gradient field, namely at optimality:
\begin{equation}
    v_t(x_t) = \nabla_{x_t} E_t(x_t)
\end{equation}

However, many dynamical systems do not evolve according to a potential field, and exhibit non gradient field dynamics. 
\subsection{ODE formulation}
Consider a set of particles drawn from source and target distributions, we are interested in finding transition trajectory between particles in the source and target distribution. Such problem can be modeled with traditional OT framework:
\begin{equation}
    \min_{q_t, v_t} \int_{0}^{1} [\frac{1}{2}\|v_t\|^{2} - U(q_t)]dt
\end{equation}
\looseness=-1
\begin{equation}
    \text{s.t} \quad \dot{q_t} = -\langle \nabla, q_tv_t \rangle, \quad v_t = \nabla E + \nabla \times B \\
    \quad \dot{q}_t = v_t
\end{equation}

\subsection{SDE formulation}
We consider data of the type predefined vector field $u(x)$, and empirical distributions $\mathcal{X}_0, \mathcal{X}_1$. Then we consider a problem of the following form
\begin{align}
    \min_v \int \frac{1}{2}\|v(x_t) - u(x_t) \|^2_2\\
    \text{s.t. } \frac{d p}{d t} = 0 \text{ and } \dot{x}_t = v(x_t)
\end{align}

most cases of stochastic optimal control consider the case where $u(x_t) = 0$.
in the stochastic case we have
\begin{align}
    \min_v \int \|v(x_t) - u(x_t) \|^2_2 + U(x_t)\\
    \text{s.t. } \frac{d p}{d t} = 0 \text{ and } \dot{x}_t = v(x_t) dt + \sigma_t dW
\end{align}
this is equivalent to non-stationary diffusion Schrodinger bridges where we consider a reference process
$x_t = u(x_t) dt + \sigma dW$.

in the non-stationary case we have
\begin{gather}
    \min_v \int \|v(x_t) - u(x_t) \|^2_2 \\
    \text{s.t. } \frac{d p_t}{d t} = \nabla \cdot (v_t  p_t) + \frac{1}{2} \sigma^2 \Delta p_t, \\
    p_0 = \mu_0, \quad p_1 = \mu_1 \quad \text{and} \quad \dot{x}_t = v(x_t) dt + \sigma_t dW
\end{gather}
by the Helmholtz decomposition we can describe $v_t$ as
\begin{equation}
    v_t = \nabla E + \nabla \times A
\end{equation}
I hypothesis that $\nabla E$ will be equal to the bridge matching vector field. Then we can describe a learning of $A$ s.t.

$\nabla \times A$ which minimizes 
\begin{gather}
    \min_A \| (\nabla E + \nabla \times A)(x_t) - u(x_t)\|_2^2 \\
    \text{ s.t. } (\nabla \times A) p_t = 0
\end{gather}

This can be combined with interacting terms and helps differentiate from GSBM and WLF. 

We have two metrics. Both the distribution matching metric but also the prior vector field matching metric. We can show equivalent performance on distribution matching while being ``more realistic'' by following the naturally defined vector field. 

\section{Schrodinger Bridge with non-zero reference field}

Given a reference process $\mathbb{Q}$ The Schr\"odinger bridge problem aims to find $\mathbb{P}^*$ which satisfies
\begin{equation}
    \mathbb{P}^* = \text{arg min} \left [ \text{KL}(\mathbb{P} | \mathbb{Q}) : \mathbb{P}_0 = \mathbb{Q}_0, \mathbb{P}_1 = \mathbb{Q}_1 \right ] 
\end{equation}
in the case of generative modelling we generally consider $\mathbb{Q}_t := \mathbb{W}_t$, i.e. $\mathbb{Q}$ has no drift term, which we denote the \textit{diffusion Schr\"odinger Bridge} problem. Computationally this can be approximated using minibatches~\cite{tong_stochastic_2024}, or using iterative Markov~\cite{shi_diffusion_2024} or proportional~\cite{bertoli_diffusion_2021} fitting. However in the more general case where $\mathbb{Q}$ is defined by the SDE:
\begin{equation}
    d X_t = f_t(X_t) dt + g_t d \mathbb{W}_t
\end{equation}
with nonzero $f_t$ existing solutions do not apply. To solve this type of Schr\"odinger bridge we will proceed in XXX steps. Given a reference process $\mathbb{Q}_t$ we will first learn the minimal conditional paths $\psi_t(x_t | x_0, x_1, \mathbb{Q}_t)$. 

\alex{Still not 100\% sure about the stochastic case. The deterministic case seems to follow through though.}
We will utilize the fact that the optimal form of $\phi_t$ is a mixture of conditional bridges, specifically, 
\begin{equation}
    \mathbb{P}_t = \mathbb{E} \psi_t(\cdot | x_0, x_1) d\pi^*(x_0, x_1)
\end{equation}
where
\begin{equation}
    \pi^* = \text{arg min}_\pi \iint c(x_0, x_1) d \pi(x_0, x_1) \text{ s.t. } \int \pi(x_0, \cdot) = q(x_0), \int \pi(\cdot, x_1) = q(x_1)
\end{equation}
and $c(x_0, x_1) = \int_0^1 \| \dot \psi_t(x_t | x_0, x_1) \|^2_2 dt$. We note that $c(x_0, x_1)$ has the unbiased stochastic estimator $c(x_0, x_1) = \frac{1}{N} \sum_{t_i} \| \dot \psi(x_t | x_0, x_1) \|^2_2$. We note that while this estimator is unbiased, this does not imply we have an unbiased estimator for $\pi^*$. Unclear if this is true. Nevertheless, this procedure may work anyway. 


First consider the case where $g_t := 0$. Then let
\begin{equation}
    \psi_t(x_t | x_0, x_1) = (1 - t) x_0 + t x_1 + (1 - t) t H_\theta(t, x_0, x_1)
\end{equation}
such that 
\begin{equation}
    \psi_t^* = \text{arg min}_\psi \int_0^1 \| \psi_t - f_t \|^2_2 dt
\end{equation}

we then mix the conditional flows according to $\pi^*$ to recover $\mathbb{P}$. 

% \xhdr{Generative Modeling via Flow-matching} 
% \begin{equation}
%     x_t = (1-t) \cdot x_0 + t \cdot x_1, \quad (x_0, x_1) \sim \pi_{x_0, x_1}
% \end{equation}

% \xhdr{Manifold flow matching} %Let $(\mathcal{M},g)$ be a smooth orientable manifold supported by a smooth map $g$, where a tangent space for a point $x$ on manifold $\mathcal{M}$ is assigned by an inner product $\langle.,.\rangle_{g}$ at $x$. We consider paths $\gamma_t$ on manifold $(\mathcal{M},g)$, which connect points $x_0$ and $x_1$ drawn from a joint distribution such that $(x_0, x_1) \sim \pi_{x_0, x_1}$.
% % \begin{equation}
% %     \gamma_t^* = \text{arg min}_{\gamma_t} \int \dot \gamma_t^T G(\gamma_t, \mathcal{D}) \dot \gamma_t dt
% % \end{equation}
% % s.t.\ $\gamma_0 = x_0$ and $\gamma_1 = x_1$.

% We consider the minimization of functionals over stochastic processes $p_t$ we have
% \begin{equation}
%     p_t^*, v_t^* = \text{arg min}_{p_t, v_t} \int V(p_t, v_t) dt
% \end{equation}
% s.t.\ $p_0 = q_0$ and $p_1 = q_1$ and the focker plank continuity equation 

% \subsection{Examples}
% \xhdr{Dynamic optimal transport} in this case we define
% \begin{equation}
% V(p_t, v_t) = \frac{1}{2}\|v_t\|^2
% \end{equation}

% \xhdr{Metric flow matching}

% \xhdr{Meta flow matching}

% % \subsection{Mean-field limit of interacting particles}

% % \begin{equation}
% %     \frac{dx}{dt} = \mathbb{E}_{p_t(y)} k(x, y), \quad \frac{\partial p_t(x)}{\partial t} = - \langle \nabla_x, p_t(x) \mathbb{E}_{p_t(y)} k(x,y) \rangle
% % \end{equation}

% % \begin{equation}
% %     V(p_t, v_t) = 
% % \end{equation}

==> NeurIPS_2025_Template/table.tex <==
\begin{table}[b]
\centering
\caption{Wasserstein-1 distance ($\downarrow$) averaged over left-out marginals for 5-dim PCA representation of single-cell data for corresponding datasets. Results are averaged over 5 independent runs.}\label{tab:5_dim}
%Results with citations are taken from corresponding papers. }
\small
 \resizebox{0.8\textwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
Method                                & Cite                   & EB                      & Multi                  \\ \midrule
% Exact OT                              & 0.831                  & 0.822                   & 0.986        \\ \midrule
Reg. CNF~\citep{finlay2020train}& ---    & 0.825\(\pm\) 0.429     & ---\\
TrajectoryNet~\citep{tong2020trajectorynet}& ---    & 0.848     & ---\\
NLSB~\citep{koshizuka2022neural}& ---    & 0.970     & ---\\ 
\midrule
DSBM~\citep{shi2023diffusion}& 1.705 \(\pm\) 0.160    & 1.775 \(\pm\) 0.429     & 1.873 \(\pm\) 0.631\\
DSB~\citep{de2021diffusion}& 0.953 \(\pm\) 0.140    & 0.862 \(\pm\) 0.023     & 1.079 \(\pm\) 0.117\\
SF\(^2\) M-Sink~\citep{tong2023simulationfree}& 1.054 \(\pm\) 0.087    & 1.198 \(\pm\) 0.342     & 1.098 \(\pm\) 0.308\\
SF\(^2\) M-Geo \citep{tong2023simulationfree} & 1.017 \(\pm\) 0.104    & 0.879 \(\pm\) 0.148     & 1.255 \(\pm\) 0.179    \\
SF\(^2\) M-Exact \citep{tong2023simulationfree} & 0.920 \(\pm\) 0.049  & 0.793 \(\pm\) 0.066     & 0.933 \(\pm\) 0.054    \\ 
\midrule
OT-CFM~\citep{tong2023improving}           & 0.882 \(\pm\) 0.058    & 0.790 \(\pm\) 0.068     & 0.937 \(\pm\) 0.054    \\
I-CFM~\citep{tong2023improving}            & 0.965 \(\pm\) 0.111    & 0.872 \(\pm\) 0.087     & 1.085 \(\pm\) 0.099    \\ 
SB-CFM~\citep{tong2023improving}           & 1.067 \(\pm\) 0.107    & 1.221 \(\pm\) 0.380     & 1.129 \(\pm\) 0.363    \\
WLF-UOT~\citep{neklyudov2023computational}& 0.733 \(\pm\) 0.063    & 0.738 \(\pm\)  0.014    & 0.911 \(\pm\) 0.147\\
WLF-SB~\citep{neklyudov2023computational} & 0.797 \(\pm\) 0.022    & 0.746 \(\pm\) 0.016    & 0.950 \(\pm\) 0.205    \\
WLF-OT~\citep{neklyudov2023computational}& 0.802 \(\pm\) 0.029    & 0.742 \(\pm\) 0.012     & 0.949 \(\pm\) 0.211\\
\midrule
% Our OT-CFM reproduction               &             0.81   \(\pm\) 0.055              &         0.7507   \(\pm\) 0.045                  &        0.9295      \(\pm\) 0.1858             \\
$\nameshort$            & 0.916 $\pm$ 0.124 & 0.822 $\pm$ 0.042 & 1.053 $\pm$ 0.095 \\
$\OTLAND$                    &      0.724   \(\pm\) 0.070               &             0.713   \(\pm\) 0.039           &        0.890   \(\pm\) 0.123                \\ 

%Bend OT-CFM  (learned wo deepset)                     &                    &                        &                        \\ 
\bottomrule
% \midrule
% WLF-(OT + potential) (\(t_{out}\) used in train)           & 0.712 \(\pm\) 0.001    & 0.651 \(\pm\) 0.002     & 0.687 \(\pm\) 0.002    \\
% WLF-(UOT + potential) (\(t_{out}\) used in train)          & 0.645 \(\pm\) 0.002    & 0.634 \(\pm\) 0.001     & 0.564 \(\pm\) 0.002    \\ \bottomrule
\end{tabular}}
%\vspace{-12pt}
\end{table}

==> macros.tex <==
\newcommand{\ah}[1]{{{\textcolor{blue}{\textbf{AH: }}}{\textcolor{orange}{#1}}}}
\newcommand{\fp}[1]{{{\textcolor{blue}{\textbf{FP: }}}{\textcolor{teal}{#1}}}}

\newcommand{\kp}[1]{{{\textcolor{blue}{\textbf{KP: }}}{\textcolor{blue}{#1}}}}

% \newcommand\ah[1]{\textcolor{red}{#1}}
\newcommand{\method}{TGR\xspace}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\newcommand{\xhdr}[1]{{\noindent\bfseries #1}.}
\hypersetup{
	colorlinks=true,       % false: boxed links; true: colored links
	linkcolor=blue,        % color of internal links
	citecolor=blue,        % color of links to bibliography
	filecolor=magenta,     % color of file links
	urlcolor=blue
}

\usepackage[framemethod=TikZ]{mdframed}
\mdfdefinestyle{MyFrame}{%
    linecolor=black,
    outerlinewidth=0.5pt,
    roundcorner=1pt,
    innertopmargin=2pt, %\baselineskip,
    innerbottommargin=2pt, %\baselineskip,
    innerrightmargin=7pt,
    innerleftmargin=7pt,
    backgroundcolor=black!0!white}

% \mdfdefinestyle{MyFrame2}{%
%     linecolor=white,
%     outerlinewidth=0.0pt,
%     roundcorner=1pt,
%     innertopmargin=0.5pt,
%     innerbottommargin=0,
%     innerrightmargin=1pt,
%     innerleftmargin=1pt,
%     backgroundcolor=black!4!white}
\mdfdefinestyle{MyFrame2}{%
    linecolor=white,
    outerlinewidth=1pt,
    roundcorner=2pt,
    innertopmargin=10pt,
    innerbottommargin=7pt,
    innerrightmargin=10pt,
    innerleftmargin=10pt,
    backgroundcolor=black!3!white}

\mdfdefinestyle{MyFrameEq}{%
    linecolor=white,
    outerlinewidth=0pt,
    roundcorner=0pt,
    innertopmargin=0pt,
    innerbottommargin=0pt,
    innerrightmargin=7pt,
    innerleftmargin=7pt,
    backgroundcolor=black!3!white}
